CryptoGuard: High Precision Detection of Cryptographic Vulnerabilities in Massive-sized Java Projects

Cryptographic API misuses, such as exposed secrets, predictable random numbers, and vulnerable certificate verification, seriously threaten software security. The vision of automatically screening cryptographic API calls in massive-sized (e.g., millions of LoC) Java programs is not new. However, hindered by the practical difficulty of reducing false positives without compromising analysis quality, this goal has not been accomplished. State-of-the-art crypto API screening solutions are not designed to operate on a large scale. Our technical innovation is a set of fast and highly accurate slicing algorithms. Our algorithms refine program slices by identifying language-specific irrelevant elements. The refinements reduce false alerts by 76% to 80% in our experiments. Running our tool, CrytoGuard, on 46 high-impact large-scale Apache projects and 6,181 Android apps generate many security insights. Our findings helped multiple popular Apache projects to harden their code, including Spark, Ranger, and Ofbiz. We also have made substantial progress towards the science of analysis in this space, including: i) manually analyzing 1,295 Apache alerts and confirming 1,277 true positives (98.61% precision), ii) creating a benchmark with 38-unit basic cases and 74-unit advanced cases, iii) performing an in-depth comparison with leading solutions including CrySL, SpotBugs, and Coverity. We are in the process of integrating CryptoGuard with the Software Assurance Marketplace (SWAMP).

==> algorithm.tex <==
\begin{algorithm*}[hb]
\caption{\textbf{\textit{calcInterProceduralSlices}} function to calculate inter-procedural backward slicing in Algorithm~\ref{code:inter-procedural}.}
\label{code:sub-procedure}
\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Input:} \texttt{criterion, methodVsAnalysis, criterionMap}
\Statex \textbf{Output:} \texttt{methodVsAnalysis}
\State \texttt{calsite} $\leftarrow$ \texttt{criterion.getCallsite()}
\State \texttt{slicingParams} $\leftarrow$ \texttt{criterion.getSlicingParams()}
\State \texttt{currMethod} $\leftarrow$ \texttt{callsite.getCaller()}

\Statex /*** Terminate if the slicingParams are empty or we already visited here. ***/

\If {\texttt{slicingParams} is empty $||$ \texttt{criterionMap.get(criterion)} $!=$ null}
\Return
\EndIf

\Statex /*** Store the criterion (with the callsite inside) to keep track whether already visited or not. ***/
\State \texttt{criterionMap.put(slicingCriteria, Boolean.TRUE)}
\Statex /*** Do intra-procedural slicing for the current method. ***/
\State \texttt{prevAnalysis} $\leftarrow$ \texttt{methodVsAnalysis.get(callsite.getCallee())}
\State \texttt{currAnalysis} $\leftarrow$ \texttt{\textbf{calcIntraProceduralSlice}(currMethod, criterion)}
\If{\texttt{currAnalysis.getUsedFields()} is not empty}

\Statex /*** Find field initializations. ***/

\For{\texttt{field} in \texttt{currAnalysis.getUsedFields()}}
\Statex /*** Find influences for the used fields. ***/
\State \texttt{listOfFieldSlicingResult} $\leftarrow$ \texttt{\textbf{calcSlicesForField}(field)}
\For{\texttt{fieldSlicingResult} in \texttt{listOfFieldSlicingResult}}
\State \texttt{containingMethod} $\leftarrow$ \texttt{fieldSlicingResult.getContainingMethod()}

\Statex /*** Concatenate fieldSlicingResult, currAnalysis and prevAnalysis. ***/
\Statex /*** Then store the result in methodVsAnalysis map by using containingMethod as the key. ***/

\State \texttt{\textbf{storeAnalysisResult}(containingMethod, fieldSlicingResult, currAnalysis, prevAnalysis, methodVsAnalysis)}
\State \texttt{callers} $\leftarrow$ \texttt{containingMethod.getCallers()}
\State \texttt{callerSites} $\leftarrow$ \texttt{getCallsites(containingMethod, callers)}
\State \texttt{newParams} $\leftarrow$ \texttt{fieldSlicingResult.getInfluencingParams()}
\Statex /*** Follow the caller chains to find field influences. ***/
\For{\texttt{newCallsite} in \texttt{callerSites}}
\State \texttt{newCriterion} $\leftarrow$ \texttt{new Criterion(newCallsite, newParams)}
\State \texttt{\textbf{calcInterProceduralSlices}(newCriterion, methodVsAnalysis, criterionMap)}
\EndFor
\EndFor
\EndFor
\EndIf
\Statex /*** Concatenate currAnalysis with prevAnalysis ***/
\Statex /*** and store the result in methodVsAnalysis map by using currMethod as the key. ***/
\State \texttt{\textbf{storeAnalysisResult}(currMethod, currAnalysis, prevAnalysis, methodVsAnalysis)}
\State \texttt{callers} $\leftarrow$ \texttt{currMethod.getCallers()}
\State \texttt{callerSites} $\leftarrow$ \texttt{getCallsites(currMethod, callers)}
\State \texttt{newParams} $\leftarrow$ \texttt{currAnalysis.getInfluencingParams()}

\Statex /*** Follow the caller chains to find parameter influences. ***/
\For{\texttt{newCallsite} in \texttt{callerSites}}
\State \texttt{newCriterion} $\leftarrow$ \texttt{new Criterion(newCallsite, newParams)}
\State \texttt{\textbf{calcInterProceduralSlices}(newCriterion, methodVsAnalysis, criterionMap)}
\EndFor

\end{algorithmic}
\end{algorithm*} 

==> android-hash.tex <==
\subsubsection{Case Study: Insecure Hash}

\begin{table}[th]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline 
\begin{tabular}[c]{@{}l@{}}Broke\\ Hash\end{tabular} & SHA & SHA1 & MD5 & MD2 \\ \hline \hline
1256                                                 & 644 & 23   & 585 & 4   \\ \hline
\end{tabular}
\caption{Broken hash frequencies among Android apps.}
\label{table:broken-hash}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline 
base packages     & counter & percent \\ \hline \hline 
com.facebook.internal  & 117     & 9.1\%  \\ \hline
com.google.firebase        & 68     & 5.3\%  \\ \hline
okio.ByteString & 66     & 5.2\%  \\ \hline
com.facebook.ads   & 62      & 4.8\%   \\ \hline
okio.Buffer          & 48 & 3.8\%  \\ \hline
\end{tabular}
\caption{The source of insecure hash functions for 326 violations. 26.9\% of them come from various libraries starting from this three base packages.}
\label{table:source-broke-hash}
\end{table}




The purpose of the case study is to understand the misuse of insecure hash functions.
Table~\ref{table:broken-hash} presents the statistics among Android applications that use insecure hash functions. we found 1256 violations in total. 46.6\% of violations are due to usage of MD5 hashing algorithm.

 MD2 is an earlier, 8-bit version of MD5. Given a message, MD2 algorithm computes 128-bit (16-byte). 
Although MD2 is insecure and vulnerable to attackers, we find the existence of MD2 in current cryptographic code implementation.
Our tool reported that \textit{io.moj.mobile.android.motion} violates the broken hash rule inside the package \url{org.apache.commons.codec.digest}. The problem is the misuse of hash function MD2 in the method \url{getSha1Digest()}. 

%To verify the result, we decompile with app and reverse engineer the source from the bytecode. The listing 1 presents the problematic method in the \url{getSha1Digest()}. 


% \begin{lstlisting}[caption= misuse of hash function MD2]
%  public static MessageDigest getDigest(String algorithm) {
%         ...
%             return MessageDigest.getInstance(algorithm);
%         ...
%     }
%     public static MessageDigest getMd2Digest() {
%         return getDigest(MessageDigestAlgorithms.MD2);
%     }
% \end{lstlisting}


Table~\ref{table:source-broke-hash} presents the packages that contain broken hash functions. Top 3 library base packages count for 326, which is 26\% of total violations. %Popular third-party libraries contain insecure code. For example, Google mobile library firebase is an embedded SDK that helps to app development and data analytics.  Inside the class \url{com.google.firebase.iid.e}, a nonsecure random function is used to initialize nonce data. 


==> fig-backups.tex <==
\begin{figure*}
\caption{A coding example to demonstrate the influence through fields. (a) \texttt{Crypto} class is used for generic AES encryption with \texttt{keyBytes}; (b) Data dependency graph of \texttt{keyBytes} variable. Here, green indicates the dependency on fields. \textbf{(Replacement for Fig 2)}}\label{coding:example}
\begin{minipage}[c]{.42\textwidth}
\begin{minipage}[c]{.42\textwidth}
\lstset{language=Java, 
   basicstyle=\ttfamily\scriptsize,
   keywordstyle=\color{blue}\ttfamily,
   stringstyle=\color{red}\ttfamily,
   commentstyle=\color{green}\ttfamily,
   morecomment=[l][\color{magenta}]{\#},
   numbers=left,
   numbersep=1pt,
   escapeinside=||,
   tabsize=1,
   firstnumber=1,
   stepnumber=1,
   showstringspaces=false,
   xleftmargin=0pt
}
\begin{lstlisting}
class Crypto {
 ...
 String defKey;

 public Crypto(String defaultKey){
  ...
  defKey = defaultKey;
 }

 byte[] encrypt(String txt){
  
  byte[] keyBytes = defKey.getBytes("UTF-8");
  ...
  SecretKeySpec keySpc =|\Suppressnumber|
         new SecretKeySpec(|\underline{keyBytes}|, ALGO);|\Reactivatenumber{15}|
  ...
 }
}
\end{lstlisting}
\end{minipage}\caption*{(a)}
\end{minipage}
\begin{minipage}[c]{.31\textwidth}
\begin{subfigure}{.999\textwidth}
 		\includegraphics[width=0.7\textwidth]{figures/property-influence.png}
 		\caption*{(b)}
        \label{program-slicing:call-graph}
 	\end{subfigure} 
\end{minipage}
\end{figure*}

\begin{figure*}
\caption{A coding example to demonstrate the influence through method parameters (a) \texttt{Crypto} class is used for generic AES encryption with \texttt{keyBytes} and \texttt{PasswordEncryptor} uses \texttt{Crypto} to encrypt passwords (b) Data dependency graph of \texttt{keyBytes} variable. Here, red indicates the dependency on method parameters. \textbf{(Replacement for Fig 2)}}\label{coding:example}
\begin{minipage}[c]{.69\textwidth}
\begin{minipage}[c]{.52\textwidth}
\lstset{language=Java, 
   basicstyle=\ttfamily\scriptsize,
   keywordstyle=\color{blue}\ttfamily,
   stringstyle=\color{red}\ttfamily,
   commentstyle=\color{green}\ttfamily,
   morecomment=[l][\color{magenta}]{\#},
   numbers=left,
   numbersep=1pt,
   escapeinside=||,
   tabsize=1,
   stepnumber=1,
   showstringspaces=false,
   xleftmargin=0pt
}

\begin{lstlisting}
class PasswordEncryptor {

 Crypto crypto;
 ...

 byte[] encPass(String pass){
  String passKey = getKey("pass.key");
  if (passKey == null){
   crypto.encrypt(pass, "enckey");
  }
  crypto.encrypt(pass, passKey);
 }
 ...
}
\end{lstlisting}
\end{minipage}
\begin{minipage}[c]{.42\textwidth}
\lstset{language=Java, 
   basicstyle=\ttfamily\scriptsize,
   keywordstyle=\color{blue}\ttfamily,
   stringstyle=\color{red}\ttfamily,
   commentstyle=\color{green}\ttfamily,
   morecomment=[l][\color{magenta}]{\#},
   numbers=left,
   numbersep=1pt,
   tabsize=1,
   escapeinside=||,
   firstnumber=12,
   stepnumber=1,
   showstringspaces=false,
   xleftmargin=0pt
}
\begin{lstlisting}
class Crypto {
 ...
 
 byte[] encrypt(String txt,String key){
 
  byte[] keyBytes = key.getBytes("UTF-8");
  ...
  SecretKeySpec keySpc =|\Suppressnumber|
         new SecretKeySpec(|\underline{keyBytes}|, ALGO);|\Reactivatenumber{20}|
  ...
 }
}
\end{lstlisting}
\end{minipage}\caption*{(a)}
\end{minipage}
\begin{minipage}[c]{.31\textwidth}
\begin{subfigure}{.999\textwidth}
 		\includegraphics[width=0.7\textwidth]{figures/argument-influence.png}
 		\caption*{(b)}
        \label{program-slicing:call-graph}
 	\end{subfigure} 
\end{minipage}
\end{figure*}

==> impl.tex <==
\section{Implementations}
\label{sec:impl}

\begin{figure}[h]
\begin{center}
\includegraphics[width=.43\textwidth]{figures/sub-project-dependency.png}
\caption{A portion of the dependency relation graph on Apache Ranger.} 
\label{sub:project-dependencies}
\end{center}
\end{figure}

In this section, we discuss the implementation details of different components of~\myname{} as presented in Figure~\ref{fig:system-design}.


{\em Sub-Project Dependency Analyzer}\label{subproject:dependency}
We consider Java projects that use \textit{gradle} or \textit{maven} as the build tool.
%After that, we perform a basic text search the usage of cryptographic APIs. We select 60 projects with the most usage of our target cryptographic APIs. Since, our analysis engine operates on binaries, we build the selected projects. 
After building the projects we parse the build scripts of each of the sub projects of a project to find the inter sub project dependencies. We build a directed acyclic graph (DAG) of a project to represent its inter sub project dependencies as shown in Figure~\ref{sub:project-dependencies}. We refer this DAG as the \textit{sub-project dependency graph}. In a sub-project dependency graph $G$, each node represents a sub-project and an edge from a node $p_i$ to another node $p_j$ represents the dependency of subproject $p_i$ on $p_j$. In Figure~\ref{sub:project-dependencies}, we show a portion of a sub-project dependency graph of Apache Ranger.

For a project, we run our analysis only for the sub-projects that have no incoming edges. We refer this type of sub-projects as \textit{root sub-projects}. In Figure~\ref{sub:project-dependencies}, \texttt{security-admin} and \texttt{plugins-kms} are two root sub-projects. Given a sub project dependency graph of a project $G$ and a root sub-project $p_1$, we can find all of its dependencies by traversing all the reachable paths from $p_1$. After that we collect all the classes of a root sub-project and its dependencies for analysis.

{\em App code distinguisher} {\bf move this somewhere later}

An APK file is bundled with all of its application code with their dependencies. So after looking into the packages from inside of an APK, it is not straightforward to separate app codes from its dependencies. We parse \texttt{AndroidManifest.xml} file to find the base package of of the app and consider all the classes with the same app base package as the app classes. We categorize other classes from app dependencies based on the similarity of their base package names.

{\em Rule Checkers.} 
 As we see in Table~\ref{table:rules}, the implementation of all of the rules requires various types program slicing. Some of the checker (Rule 4 and 5) first identifies a target method definition and run intra-procedural backward program slicing to screen the method definition. The checker for Rule 6 uses forward program slicing to determine whether a socket is manually checked to have proper host name. Checker of Rule 14 also uses forward program slicing to determine whether an explicit call to \texttt{initialize} method is used to set the key size of an asymmetric cipher. Other checkers uses inter-procedural backward program slicing to find the influences to the rule specific point of interests. Then the slices are analyzed to examine whether the program complies with the rules or not. 
 
We present the implementation details and the slicing criteria of our rule checkers in Appendix B.



==> introduction.bk.tex <==
\section{Introduction}

\textbf{Sazzadur, please try to complete the introduction by this Wednesday. keep it short. also read my new title and new abstract.}

\begin{itemize}
\item First discuss the dangers of API Misuse
\item Discuss the dangers of hardcoding keys and passwords (also the right ways to do it).
\item Discuss existing tools and limitations
\item Discuss How \myname{} overcomes the limitations (Highlight Soundness and Heuristics).
\end{itemize}

Software vulnerabilities are costly. NIST estimates that cost to be \$60 billion each year, which includes the costs for developing and distributing software patches and reinstalling infected systems and the lost productivity due to malware and other software errors~\cite{software-error-cost}. The problem of software vulnerabilities is not new. What is new (and promising) is the increasing adoption of cryptography and security mechanisms in common software applications. This increase may be due to the improved security awareness in the industry, as well as stricter government regulations (e.g., in healthcare and finance domains). 

% following paragraph seems like a distraction

% However, it is difficult to write cryptographic code correctly~\cite{***}. For the software industry, the practical task of securing cryptographic implementation (at both the library-level and the application) is still in its infancy. This status is in sharp contrast with the multi-decade theoretical advancement of modern cryptography. This gap becomes particularly alarming, after multiple  recent high-profile discoveries of cryptography-related vulnerable code in widely used network libraries and tools~\cite{USENIX-Security-iMessage-2016,DBLP:conf/ccs/AdrianBDGGHHSTV15,DBLP:conf/ccs/CheckowayMGFC0H16}.

Existing research related to cryptographic implementations falls into two main categories, {\em i)}  studies to understand the current practices~\cite{SP-crypto-API-2017,Bodden-crypto-API-2015,Survey-SecDev-2017,Na-Meng-stackoverflow,DBLP:conf/sp/AcarBFKMS16} and {\em ii)}  studies to expose vulnerabilities (e.g.,~\cite{DBLP:conf/ccs/EgeleBFK13,DBLP:conf/ccs/GeorgievIJABS12, DBLP:conf/sp/SivakornAPKJ17,DBLP:conf/ccs/NguyenWABWF17,DBLP:conf/uss/RuiterP15, DBLP:conf/nsdi/ChiCNRS17}). 
%
Several coding user studies, some of which involved professional developers, have revealed serious deficiencies in coding with cryptographic APIs. For example, researchers concluded that developers need easy-to-use code examples (e.g., copyable code snippet)~\cite{SP-crypto-API-2017,Survey-SecDev-2017}. Developers expressed the need for task-oriented code examples, as existing description-based documentation is time-consuming to read and not helpful~\cite{SP-crypto-API-2017,Bodden-crypto-API-2015}. 

Developers mistakenly believe they have achieved security, specifically 78 of 396 tasks (19.7\%) fell into this category in a recent study~\cite{SP-crypto-API-2017}. In addition, virtually all the empirical studies show a serious lack of cryptography/security training in developers (e.g.,~\cite{DBLP:journals/corr/abs-1709-09970}). This finding further validates the importance of automatic code screening. 

The state-of-the-art detection approaches against cryptographic vulnerabilities are mostly 
***

dynamic, requiring the concrete execution of the program. A common approach is fuzzing (e.g.,~\cite{DBLP:conf/ccs/GeorgievIJABS12,DBLP:conf/sp/SivakornAPKJ17}). Blackbox fuzzing analysis approaches are relatively straightforward. It was used for verifying hostname verification~\cite{DBLP:conf/sp/SivakornAPKJ17} and certificate validation in SSL/TLS~\cite{DBLP:conf/ccs/GeorgievIJABS12}. 
Another notable dynamic approach is to validate runtime protocol behaviors with a verifier, which is capable of detecting invalid or inconsistent network messages~\cite{DBLP:conf/nsdi/ChiCNRS17}. Although the work in~\cite{DBLP:conf/nsdi/ChiCNRS17} uses static symbolic execution to infer client behaviors, it requires the concrete execution of programs for detecting anomalies. 

However, fuzzing cannot detect subtle vulnerabilities that do not manifest themselves in simple observable behaviors (i.e., not externally observable). Examples of such cryptographic violations include the use of improper IVs in ciphers, poor random number generation, the leak of secrets, or the use of legacy cryptographic primitives. The aforementioned solutions can only find input guided vulnerabilities with externally visible behaviors (e.g., ***\cite{DBLP:conf/sp/SivakornAPKJ17}, program crashes~\cite{DBLP:conf/ccs/Somorovsky16} or anomalous protocol states~\cite{DBLP:conf/uss/RuiterP15, DBLP:conf/nsdi/ChiCNRS17}). 
In addition, fuzzing and other dynamic analysis techniques typically cannot guarantee coverage, which may result in missed detection~\cite{DBLP:conf/sp/ChauCHGKNL17}.  

The complementary approach of static analysis has the potential to provide better code coverage and scalability. Unlike blackbox fuzzing, static analysis requires the access to the source code or some intermediate representations of the binaries. However, most of the existing static analysis tools are  designed to demonstrate vulnerabilities, as opposed to be used as a rigorous screening tool with soundness and security guarantees. 
For example, the static analysis tool {\sc CryptoLint} was used in an empirical study to expose cryptographic misuses in Android applications (such as hardcoded keys)~\cite{DBLP:conf/ccs/EgeleBFK13}. 

The recent FixDroid  is an IDE plugin for helping Android developers write secure code~\cite{DBLP:conf/ccs/NguyenWABWF17}. FixDroid, built on the program structure index of Intellij IDEA platform,  provides localized static code analysis and is designed to analyze code snippets in isolation. 

soundness

%A sound static analysis overapproximates the behaviors of the program. A sound static analyzer is guaranteed to identify all violations of our property φ, but may also report some “false alarms”, or violations of φ that cannot actually occur. 
%
%A complete static analysis underapproximates the behaviors of the program. Any violation of our property φ reported by a complete static analyzer corresponds to an actual violation of φ, but there is no guarantee that all actual violations of φ will be reported

\myname is an automatic tool that verifies Java programs  cryptography code development.~\footnote{Sazzadur, explain hestia, the name.} 
Cryptographic program analysis (CPA) maps cryptographic properties of a program to rules that can be enforced through static program analysis methods. It provides an effective and easy-to-deploy compile-time code checking mechanism that can drastically improve the software assurance. 
We demonstrate the use of static program analysis for detecting a set of cryptographic implementation vulnerabilities.


{\bf Sazzadur, these bullet points are the key. highlight experimental findings. thanks.}

Our contributions are summarized as follows.

\begin{enumerate}
\item
several new analysis mechanisms for security.

broader collection of APIs
% setSeed()

A straightforward analysis approach may generate false positives, i.e., program slices that are returned by an analysis, however, do not correspond to vulnerable code. We address the challenge of how to reduce false positives, without causing missed detections. 
 
- Forward slicing,

% Rigors of analysis 

\item
security coverage

\item
- Data science project 
- accuracy reports. 
- Comparison with FixDroid

\end{enumerate}


==> listingbackup.tex <==
\begin{figure*}
\begin{minipage}[c]{.47\textwidth}
\lstset{language=Java, 
   basicstyle=\ttfamily\footnotesize,
   keywordstyle=\color{blue}\ttfamily,
   stringstyle=\color{red}\ttfamily,
   commentstyle=\color{green}\ttfamily,
   morecomment=[l][\color{magenta}]{\#},
   numbers=left,
   numbersep=1pt,
   tabsize=1,
   stepnumber=1,
   showstringspaces=false,
   xleftmargin=0pt
}
\begin{lstlisting}[title={(a)}]
 
 <http:tlsClientParameters disableCNCheck="true">
         ...
 </http:tlsClientParameters>

\end{lstlisting}
\begin{lstlisting}[title={(b)}]
...
        
} else if (tlsClientParameters.isDisableCNCheck()) {
   verifier = new AllowAllHostnameVerifier();
}
...
        
\end{lstlisting}
%A portion of https-cfg-client.xml in Cxf that disables hostname verification checks.
%A portion of SSLUtils.java in Cxf that allows all hostnames.
\end{minipage}
\begin{minipage}[c]{.47\textwidth}
\lstset{language=Java, 
   basicstyle=\ttfamily\footnotesize,
   keywordstyle=\color{blue}\ttfamily,
   stringstyle=\color{red}\ttfamily,
   commentstyle=\color{green}\ttfamily,
   morecomment=[l][\color{magenta}]{\#},
   numbers=left,
   numbersep=1pt,
   tabsize=1,
   firstnumber=22,
   stepnumber=1,
   showstringspaces=false,
   xleftmargin=0pt
}
\begin{lstlisting}[caption={A portion of UpsServices.java in Ofbiz that allow trusting all certificates.},captionpos=b]

public static String sendUpsRequest(...) {
  ...
  HttpClient http = new HttpClient(conStr);
  http.setTimeout(timeout * 1000);
  http.setAllowUntrusted(true);
  ...
}
\end{lstlisting}
\begin{lstlisting}[caption={A portion of SSLUtil.java in Ofbiz that uses a dummy trust manager.},captionpos=b]

SSLContext getSSLContext(String alias, 
                         boolean trustAny) {
   ...  
   TrustManager[] tm;
   if (trustAny) {
      tm = SSLUtil.getTrustAnyManagers();
   } else {
      tm = SSLUtil.getTrustManagers();
   }
   ...
}
\end{lstlisting}
\end{minipage}
\caption{Coding example of disabling Hostname verification (Listing 1 and 2) and trusting all certificates (Listing 3 and 4)}\label{example:rule45}
\end{figure*}

==> projectlist.tex <==
\subsection{Project List}

 482 Apache projects are hosted in github, those have Java as one of the language. 82 of them uses \texttt{Cipher.getInstance}. 181 projects uses \texttt{MessageDigest.getInstance}. In total 195 projects use both of them.
 
 \begin{table*}[!ht]
 	\caption{Project List vs Vulnerability.}
 	\begin{normalsize}
 	\begin{tabular}{|>{\xsmall}m{0.5cm}|>{\xsmall}m{1.5cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|>{\xsmall}m{0.3cm}|}
 		\hline
 		 Serial & Project & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\
 		\hline \hline
 		 1 & ambari & - & - & - & - & - & - & - & - & - & - & - & - & \xmark & - & - & -  \\
         \hline
         2 & ranger & - & - & - & - & - & \xmark & - & - & - & - & - & - & \xmark & - & - & \xmark  \\
         \hline
         3 & sling & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & \xmark  \\
         \hline
         4 & ofbiz & - & \xmark & - & - & - & - & - & - & - & - & - & - & - & - & - & \xmark  \\
 		\bottomrule
 	\end{tabular}
 	\end{normalsize}
 \end{table*}

==> rules.bk.tex <==
\section{Security Rules}
\input{table}

Add rules related to privacy oracle. [looks like unrelated]
\url{https://homes.cs.washington.edu/~yoshi/papers/PrivacyOracle/privacyoracle-ccs2008.pdf}

Expand cases from prof. Na Meng's work (Section 4.3 of submitted manuscript in ICSE).


Include the rules related to the SSL validation API misuses. See the following Papers: 
	1.The most dangerous code in the world: validating SSL certificates in non-browser software.
    2. \url{https://www.luis.uni-hannover.de/fileadmin/it_sicherheit/pdf/SiTaWS1213_Android_Apps.pdf}
    3. \url{https://www.codeproject.com/Articles/826045/Android-security-Implementation-of-Self-signed-SSL}
    4. \url{https://www.cert.org/vulnerability-analysis/tools/cert-tapioca.cfm}
    5. \url{https://developer.android.com/training/articles/security-ssl.html}



==> threatmodel.tex <==
\section{Threat Model}
